The Quantum Pendulum of Turbulent Flow: Decaying turbulence as a thermal state of an integrable system

We present a theory of decaying turbulence in which the statistics of a classical flow becomes quantum mechanics in loop space. The loop functional plays the role of a wave function, and the Navier-Stokes equation makes it evolve linearly, with the viscosity as Planck constant. Turbulence at infinite Reynolds number is defined by a discretized loop equation on polygons with $N$ sides and a renormalization. It has an exact manifold of decaying solutions, the Euler ensemble; each is a singular point of the deterministic equation, which does not select their weights. We interpret this instability as the source of spontaneous stochasticity: thermal noise only triggers a diffusion of the momentum loop over the Euler states, and neither its amplitude nor the temperature of the fluid enters the statistics. In a stochastic model of this diffusion equal weights are proved to be the attractor. As a fermion trace, the partition function and the vorticity correlations become Gibbs averages of two quantum pendulums with the Mathieu Hamiltonian. The energy spectrum is a chain of explicit quadratures. It falls as $k^{-7/2}$ at large $k$; at $kL=\sqrt{2}$, with $L=\sqrt{\tilde\nu(t+t_0)}$, its slope diverges as a double logarithm, so the decay at a fixed wave number is singular at a finite time and the vorticity correlation oscillates. At small $k$ there are two solutions, for a quenched and an annealed orientation of the plane of the loop: $k^{-1}\log(1/kL)$ and $k^{-2}/\log(1/kL)$. The energy and its dissipation depend on the size of the system logarithmically in the first and almost linearly in the second, and the energy decays with an index of 1.1-1.2 and about 1.45. The reduction to the quantum pendulum is formally verified in Lean 4 in a forthcoming paper. The theory rests on stated physical hypotheses; its comparison with simulations and experiment is left to a separate paper.

==> xref/Supplement_labels.tex <==
% Labels regenerated from Supplement.aux (anchor and file fields blank).
% Revision (ab) of 2026-11-16: regenerated; no number changed.
\makeatletter
\newlabel{sec:S-intro-details}{{S1}{4}{The Introduction: details}{}{}}
\newlabel{rem:intro-positivity}{{S1.1}{6}{}{}{}}
\newlabel{sec:S-mle}{{S2}{10}{The momentum-loop equation: details}{}{}}
\newlabel{eq:physical-ns-vector}{{S2.1}{10}{The momentum-loop equation: details}{}{}}
\newlabel{sec:S-mle-proofs}{{S2.1}{11}{The operator identity and the calculus of jumps}{}{}}
\newlabel{eq:qsp-pexp}{{S2.2}{11}{The operator identity}{}{}}
\newlabel{eq:qsp-transport}{{S2.3}{11}{The operator identity}{}{}}
\newlabel{sec:S-qsp-examples}{{S3}{13}{The Quantum Statistical Principle: the correspondence and the examples}{}{}}
\newlabel{sec:S-qsp-correspondence}{{S3.1}{13}{Classical statistics and quantum mechanics}{}{}}
\newlabel{sec:qsp-gibbs}{{S3.2}{13}{The Gibbs distribution}{}{}}
\newlabel{eq:qsp-thermal}{{S3.1}{13}{The Gibbs distribution}{}{}}
\newlabel{eq:qsp-perimeter}{{S3.2}{14}{The Gibbs distribution}{}{}}
\newlabel{eq:qsp-white}{{S3.3}{14}{The Gibbs distribution}{}{}}
\newlabel{eq:qsp-gibbs-field}{{S3.4}{14}{The operator form}{}{}}
\newlabel{eq:qsp-gibbs-displacement}{{S3.5}{14}{The operator form}{}{}}
\newlabel{eq:qsp-gibbs-W}{{S3.6}{14}{Proper time}{}{}}
\newlabel{sec:qsp-rotation}{{S3.3}{15}{The uniform rotation}{}{}}
\newlabel{eq:qsp-rotation}{{S3.7}{15}{The uniform rotation}{}{}}
\newlabel{eq:qsp-rotation-loop}{{S3.8}{15}{The uniform rotation}{}{}}
\newlabel{eq:qsp-rotation-correlator}{{S3.9}{15}{The uniform rotation}{}{}}
\newlabel{eq:qsp-rotation-action}{{S3.10}{15}{Quantization}{}{}}
\newlabel{eq:qsp-rotation-commutator}{{S3.11}{15}{Quantization}{}{}}
\newlabel{eq:qsp-oscillator}{{S3.12}{15}{Quantization}{}{}}
\newlabel{eq:qsp-holonomy}{{S3.13}{16}{The exact trace}{}{}}
\newlabel{eq:qsp-ordered}{{S3.14}{16}{The state}{}{}}
\newlabel{eq:qsp-vorticity}{{S3.15}{16}{Vorticity as a commutator}{}{}}
\newlabel{sec:qsp-rotating}{{S3.4}{17}{The rotating fluid in thermal equilibrium}{}{}}
\newlabel{eq:qsp-rotating}{{S3.16}{17}{The rotating fluid in thermal equilibrium}{}{}}
\newlabel{eq:qsp-rotating-P}{{S3.17}{17}{The rotating fluid in thermal equilibrium}{}{}}
\newlabel{sec:S-qsp-euler}{{S3.5}{17}{The Euler ensemble in the language of the principle}{}{}}
\newlabel{sec:qsp-stochasticity}{{S3.6}{18}{A representation suited to spontaneous stochasticity}{}{}}
\newlabel{sec:S-qsp}{{S4}{19}{The Quantum Statistical Principle: details}{}{}}
\newlabel{eq:S-qsp-area}{{S4.1}{19}{The area tensor of a polygon}{}{}}
\newlabel{eq:S-qsp-area-identities}{{S4.2}{19}{The area tensor of a polygon}{}{}}
\newlabel{eq:S-qsp-cot}{{S4.3}{19}{Antiperiodic modes}{}{}}
\newlabel{eq:S-qsp-modes}{{S4.4}{19}{Antiperiodic modes}{}{}}
\newlabel{eq:S-qsp-halfinteger}{{S4.5}{19}{Antiperiodic modes}{}{}}
\newlabel{eq:S-qsp-bch}{{S4.6}{20}{The ordered product}{}{}}
\newlabel{sec:bv-sphere}{{S5}{21}{Jumps, the sphere, and the spherical-sector postulate}{}{}}
\newlabel{eq:spherical-telescoping}{{S5.1}{22}{Spherical confinement}{}{}}
\newlabel{eq:diffusive-stationary-geometry}{{S5.2}{22}{Spherical confinement}{}{}}
\newlabel{sec:S-bv}{{S6}{22}{The calculus of jumps}{}{}}
\newlabel{eq:variation-divergence}{{S6.1}{23}{The calculus of jumps}{}{}}
\newlabel{sec:S-contact}{{S7}{23}{The second area derivative: derivation}{}{}}
\newlabel{eq:ct-tangent}{{S7.1}{23}{The second area derivative: derivation}{}{}}
\newlabel{eq:ct-area-operator}{{S7.2}{23}{The second area derivative: derivation}{}{}}
\newlabel{eq:ct-chain}{{S7.3}{23}{The second area derivative: derivation}{}{}}
\newlabel{eq:ct-product}{{S7.4}{24}{The second area derivative: derivation}{}{}}
\newlabel{eq:ct-product-fixed}{{S7.5}{24}{The second area derivative: derivation}{}{}}
\newlabel{eq:ct-kick}{{S7.6}{24}{The second area derivative: derivation}{}{}}
\newlabel{sec:S-ct-polygon}{{S7.1}{25}{The polygon: the pair weight and the normalization}{}{}}
\newlabel{eq:ct-polygon}{{S7.7}{25}{The polygon: the pair weight and the normalization}{}{}}
\newlabel{eq:ct-normalized}{{S7.8}{25}{The normalization}{}{}}
\newlabel{sec:S-contact-main}{{S7.2}{25}{The rule at the mark, the invariances and the diagonal}{}{}}
\newlabel{sec:S-contact-image}{{S7.3}{27}{The momentum image, step by step}{}{}}
\newlabel{eq:S-contact-composition}{{S7.9}{27}{Step 1: the composition is the second area derivative}{}{}}
\newlabel{eq:S-contact-gradient-coord}{{S7.10}{28}{Step 3: one gradient insertion}{}{}}
\newlabel{eq:S-contact-product}{{S7.11}{28}{Step 5: the product of the two insertions}{}{}}
\newlabel{eq:S-contact-op}{{S7.12}{29}{Step 7: the rule at the mark}{}{}}
\newlabel{eq:S-contact-ordered}{{S7.13}{29}{Step 7: the rule at the mark}{}{}}
\newlabel{sec:S-contact-rotation}{{S7.4}{30}{Benchmark: the uniform rotation}{}{}}
\newlabel{eq:S-contact-rot-cov}{{S7.14}{30}{Representation and convention}{}{}}
\newlabel{eq:S-contact-rot-sawtooth}{{S7.15}{30}{Representation and convention}{}{}}
\newlabel{eq:S-contact-refined-F}{{S7.16}{30}{Refinement conventions}{}{}}
\newlabel{eq:S-contact-rot-pairs}{{S7.17}{31}{Without refinement}{}{}}
\newlabel{eq:S-contact-rot-totals}{{S7.18}{31}{Without refinement}{}{}}
\newlabel{lem:S-contact-local}{{S7.1}{32}{Local bounds on the terms at the mark}{}{}}
\newlabel{eq:S-contact-local}{{S7.19}{32}{Local bounds on the terms at the mark}{}{}}
\newlabel{eq:S-contact-adj}{{S7.20}{33}{The Euler states}{}{}}
\newlabel{rem:S-contact-locations}{{S7.2}{33}{Typical locations}{}{}}
\newlabel{sec:two-dimensional}{{S8}{34}{Two dimensions: the complex rotating polygon}{}{}}
\newlabel{eq:2d-rescaling}{{S8.1}{34}{Two dimensions: the complex rotating polygon}{}{}}
\newlabel{eq:2d-full-rescaled}{{S8.2}{34}{Two dimensions: the complex rotating polygon}{}{}}
\newlabel{eq:2d-arithmetic-parameters}{{S8.3}{34}{Rational angles and the logarithmic rotation}{}{}}
\newlabel{prop:2d-complex-rotation}{{S8.1}{35}{Complex planar Euler trajectory}{}{}}
\newlabel{eq:2d-complex-rotation}{{S8.4}{35}{Complex planar Euler trajectory}{}{}}
\newlabel{eq:2d-invariants}{{S8.5}{35}{Complex planar Euler trajectory}{}{}}
\newlabel{eq:2d-complex-phase-average}{{S8.6}{35}{A real representative of the orientation average}{}{}}
\newlabel{prop:2d-phase-shift}{{S8.2}{35}{Moving the orientation contour}{}{}}
\newlabel{eq:2d-real-phase-average}{{S8.7}{35}{Moving the orientation contour}{}{}}
\newlabel{sec:two-dimensional-rigidity}{{S9}{36}{Two dimensions: rigidity on the circle}{}{}}
\newlabel{eq:2d-angle-gaps}{{S9.1}{36}{Two dimensions: rigidity on the circle}{}{}}
\newlabel{prop:2d-fixed-circle-rigidity}{{S9.1}{36}{Local rigidity of real gaps}{}{}}
\newlabel{sec:2d-positivity}{{S10}{36}{Two dimensions: the vorticity correlation violates positivity}{}{}}
\newlabel{eq:2d-polygon-spectrum}{{S10.1}{36}{Two dimensions: the vorticity correlation violates positivity}{}{}}
\newlabel{eq:2d-two-insertion-sign}{{S10.2}{37}{Two dimensions: the vorticity correlation violates positivity}{}{}}
\newlabel{eq:2d-corrected-pair}{{S10.3}{37}{Two dimensions: the vorticity correlation violates positivity}{}{}}
\newlabel{eq:2d-zero-separation}{{S10.4}{37}{Two dimensions: the vorticity correlation violates positivity}{}{}}
\newlabel{prop:2d-rejected}{{S10.1}{37}{The planar solution fails the finite-cutoff enstrophy test}{}{}}
\newlabel{sec:2d-cond}{{S10.1}{38}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-Q}{{S10.5}{38}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-mid}{{S10.6}{38}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-split}{{S10.7}{38}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-zero}{{S10.8}{39}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-neumann}{{S10.9}{39}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-limit}{{S10.10}{39}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-asym}{{S10.11}{39}{The conditional correlation}{}{}}
\newlabel{prop:2d-conditional}{{S10.2}{40}{The conditional correlation of the planar solution is negative}{}{}}
\newlabel{eq:2d-cond-transforms}{{S10.12}{40}{The conditional correlation}{}{}}
\newlabel{eq:2d-cond-measure}{{S10.13}{41}{The conditional correlation}{}{}}
\newlabel{sec:S-2d}{{S11}{41}{Two dimensions: the complex rotation, its average and the conditional correlation}{}{}}
\newlabel{eq:2d-stretch}{{S11.1}{41}{Two dimensions: the complex rotation, its average and the conditional correlation}{}{}}
\newlabel{rem:2d-growth}{{S11.2}{42}{Where the growth goes}{}{}}
\newlabel{eq:2d-growth-z}{{S11.2}{42}{Where the growth goes}{}{}}
\newlabel{eq:2d-growth-J0}{{S11.3}{42}{Where the growth goes}{}{}}
\newlabel{sec:S-2d-cond}{{S11.1}{43}{The conditional correlation: derivations and numbers}{}{}}
\newlabel{eq:S-2d-marks}{{S11.4}{43}{The phases at the marks for any polygon}{}{}}
\newlabel{eq:S-2d-mellin}{{S11.5}{45}{The Mellin transforms and the asymptotes}{}{}}
\newlabel{eq:S-2d-F}{{S11.6}{46}{Positive values at finite $N$}{}{}}
\newlabel{sec:S-2d-rigidity}{{S12}{47}{Two dimensions: proof of rigidity on the circle}{}{}}
\newlabel{eq:2d-gap-equation}{{S12.1}{47}{Two dimensions: proof of rigidity on the circle}{}{}}
\newlabel{eq:2d-phase-equation}{{S12.2}{47}{Two dimensions: proof of rigidity on the circle}{}{}}
\newlabel{eq:2d-gap-derivatives}{{S12.3}{48}{Two dimensions: proof of rigidity on the circle}{}{}}
\newlabel{eq:2d-linear-difference}{{S12.4}{48}{The formal square mode}{}{}}
\newlabel{eq:2d-linear-sum}{{S12.5}{48}{The formal square mode}{}{}}
\newlabel{eq:2d-formal-square-mode}{{S12.6}{48}{The formal square mode}{}{}}
\newlabel{eq:2d-square-obstruction}{{S12.7}{48}{The formal square mode}{}{}}
\newlabel{eq:2d-varying-square}{{S12.8}{48}{A fixed radius is stronger than a varying one}{}{}}
\newlabel{sec:S-3d-odd}{{S13}{49}{Three dimensions: the odd states and the counting measure}{}{}}
\newlabel{eq:3d-all-winding-collapse}{{S13.1}{49}{Three dimensions: the odd states and the counting measure}{}{}}
\newlabel{eq:3d-exact-all-winding-Z}{{S13.2}{49}{Three dimensions: the odd states and the counting measure}{}{}}
\newlabel{sec:3d-grand}{{S14}{49}{Three dimensions: the grand canonical ensemble and the dominance of zero winding}{}{}}
\newlabel{eq:grand-ratio}{{S14.1}{50}{Three sectors}{}{}}
\newlabel{sec:S-3d}{{S15}{51}{Three dimensions: the real phase representative and the counting}{}{}}
\newlabel{sec:S-3d-real}{{S15.1}{52}{The real phase representative and its scope}{}{}}
\newlabel{eq:3d-real-phase}{{S15.2}{52}{The real phase representative and its scope}{}{}}
\newlabel{sec:S-3d-main}{{S15.2}{52}{The statistical weight: invariance and the limit}{}{}}
\newlabel{sec:rigidity3d}{{S16}{53}{Three dimensions: rigidity of the odd and even Euler ensembles}{}{}}
\newlabel{eq:rig3d-fixed-lift}{{S16.1}{53}{Rigidity of the complex Euler polygon}{}{}}
\newlabel{prop:rig3d}{{S16.1}{53}{Rigidity of the fixed complex lift}{}{}}
\newlabel{prop:rig3d-even}{{S16.2}{53}{Rigidity of the fixed complex lift for even $N$}{}{}}
\newlabel{rem:rig3d-family}{{S16.3}{54}{The family of zero-winding fixed points}{}{}}
\newlabel{rem:rig3d-linear}{{S16.4}{54}{The unrestricted linearization}{}{}}
\newlabel{eq:rig3d-invariant-measure}{{S16.2}{55}{Invariance of the selected ensemble}{}{}}
\newlabel{sec:S-3d-rigidity}{{S17}{55}{Three dimensions: proofs of rigidity}{}{}}
\newlabel{eq:rig3d-operators}{{S17.1}{55}{Three dimensions: proofs of rigidity}{}{}}
\newlabel{eq:rig3d-rescaling}{{S17.2}{55}{Three dimensions: proofs of rigidity}{}{}}
\newlabel{eq:rig3d-inverse}{{S17.3}{55}{Three dimensions: proofs of rigidity}{}{}}
\newlabel{eq:rig3d-complex-defects}{{S17.4}{55}{Three dimensions: proofs of rigidity}{}{}}
\newlabel{eq:rig3d-null-reduction}{{S17.5}{56}{Three dimensions: proofs of rigidity}{}{}}
\newlabel{eq:rig3d-normal-equation}{{S17.6}{56}{Three dimensions: proofs of rigidity}{}{}}
\newlabel{sec:S-rig3d-even}{{S17.1}{56}{Even \texorpdfstring {$N$}{N}}{}{}}
\newlabel{eq:rig3d-real-rescaled}{{S17.7}{56}{Exact angular compatibility of the real diffusive representative}{}{}}
\newlabel{eq:rig3d-circle-angles}{{S17.8}{56}{Exact angular compatibility of the real diffusive representative}{}{}}
\newlabel{eq:rig3d-angular-midpoint}{{S17.9}{56}{Exact angular compatibility of the real diffusive representative}{}{}}
\newlabel{eq:rig3d-angular-compatibility}{{S17.10}{57}{Exact angular compatibility of the real diffusive representative}{}{}}
\newlabel{eq:rig3d-linear-compatibility}{{S17.11}{57}{Exact angular compatibility of the real diffusive representative}{}{}}
\newlabel{eq:rig3d-angular-pencil}{{S17.12}{57}{Exact angular compatibility of the real diffusive representative}{}{}}
\newlabel{eq:rig3d-even-period-two}{{S17.13}{57}{Even $N$, real representative}{}{}}
\newlabel{sec:rig3d-neutral}{{S17.3}{57}{Radial directions, spherical confinement, and neutral shapes}{}{}}
\newlabel{eq:rig3d-telescopic-bound}{{S17.14}{57}{Radial directions, spherical confinement, and neutral shapes}{}{}}
\newlabel{eq:rig3d-time-origin}{{S17.15}{58}{Radial directions, spherical confinement, and neutral shapes}{}{}}
\newlabel{eq:rig3d-coupled-defects}{{S17.16}{58}{Radial directions, spherical confinement, and neutral shapes}{}{}}
\newlabel{sec:S-hairpin}{{S18}{58}{Three dimensions: the vorticity correlation, details}{}{}}
\newlabel{rem:3d-normal-only}{{S18.1}{58}{The normal component and the earlier calculations}{}{}}
\newlabel{eq:3d-unrestricted-cot-square}{{S18.1}{59}{Zero separation in the odd ensemble}{}{}}
\newlabel{eq:3d-binomial-moment-identities}{{S18.2}{59}{Zero separation in the odd ensemble}{}{}}
\newlabel{eq:3d-YN}{{S18.3}{59}{Zero separation in the odd ensemble}{}{}}
\newlabel{rem:S-small-angles}{{S18.2}{60}{Why the small angles of Ref.~\cite {migdal2024quantum} do not contribute}{}{}}
\newlabel{sec:S-cond-remarks}{{S19}{61}{The conditional correlation: the hairpin amplitude, the literal ratio and other orders}{}{}}
\newlabel{sec:hairpin-not-one}{{S19.1}{61}{The hairpin factor is not one}{}{}}
\newlabel{eq:hp-stokes}{{S19.1}{61}{Coordinate space}{}{}}
\newlabel{eq:hp-phase}{{S19.2}{62}{Momentum space}{}{}}
\newlabel{sec:S-cond-translation}{{S19.2}{62}{The planar vorticity is a translation}{}{}}
\newlabel{sec:S-cond-bulk}{{S19.3}{62}{The literal ratio and the bulk of the hairpin}{}{}}
\newlabel{eq:cond-bulk-mid}{{S19.3}{62}{The literal ratio and the bulk of the hairpin}{}{}}
\newlabel{sec:S-cond-factorization}{{S19.4}{63}{A heuristic factorization}{}{}}
\newlabel{eq:cond-factorization}{{S19.4}{63}{A heuristic factorization}{}{}}
\newlabel{sec:S-cond-orders}{{S19.5}{63}{The other orders of the averages}{}{}}
\newlabel{eq:cond-def-r}{{S19.5}{63}{The other orders of the averages}{}{}}
\newlabel{sec:S-cond-odd-zero}{{S19.6}{64}{The odd ensemble at zero separation}{}{}}
\newlabel{sec:S-hairpin-main}{{S20}{65}{The vorticity correlation: closure sums, the hairpin factor and the finite-\texorpdfstring {$N$}{N} ratio}{}{}}
\newlabel{sec:S-hp-closure}{{S20.1}{65}{The contraction, the conventions, the pair weight and the Hankel inversion}{}{}}
\newlabel{eq:3d-vorticity-contraction}{{S20.1}{65}{The contraction, the conventions, the pair weight and the Hankel inversion}{}{}}
\newlabel{eq:3d-closure-sums}{{S20.2}{65}{The contraction, the conventions, the pair weight and the Hankel inversion}{}{}}
\newlabel{eq:3d-pair-weight}{{S20.3}{65}{The contraction, the conventions, the pair weight and the Hankel inversion}{}{}}
\newlabel{eq:3d-vorticity-correlation}{{S20.4}{66}{The contraction, the conventions, the pair weight and the Hankel inversion}{}{}}
\newlabel{eq:3d-hankel-inversion}{{S20.5}{66}{The contraction, the conventions, the pair weight and the Hankel inversion}{}{}}
\newlabel{sec:S-hp-factor}{{S20.2}{66}{The hairpin factor: the bound, the variance and the values}{}{}}
\newlabel{sec:S-hp-finiteN}{{S20.3}{67}{The conditional correlation at finite \texorpdfstring {$N$}{N}}{}{}}
\newlabel{eq:3d-formal-dissipation}{{S20.6}{67}{The pendulum limit}{}{}}
\newlabel{sec:3d-transfer}{{S21}{68}{Three dimensions: an exact transfer-matrix formula}{}{}}
\newlabel{eq:3d-transfer-marks}{{S21.1}{68}{Three dimensions: an exact transfer-matrix formula}{}{}}
\newlabel{eq:3d-transfer-formula}{{S21.2}{68}{Three dimensions: an exact transfer-matrix formula}{}{}}
\newlabel{sec:S-fermion-main}{{S22}{68}{The fermionic trace: derivations, quantum thimbles and the chain of representations}{}{}}
\newlabel{eq:fermion-markov}{{S22.1}{69}{The Markov product and the counting}{}{}}
\newlabel{eq:fermion-markov-product}{{S22.2}{69}{The Markov product and the counting}{}{}}
\newlabel{eq:fermion-sector-average}{{S22.3}{69}{The Markov product and the counting}{}{}}
\newlabel{sec:S-fermion-transfer}{{S22.3}{69}{The transfer operator at a rational angle}{}{}}
\newlabel{eq:fermion-insertion}{{S22.4}{69}{The transfer operator at a rational angle}{}{}}
\newlabel{eq:fermion-two-spin}{{S22.5}{70}{The transfer operator at a rational angle}{}{}}
\newlabel{eq:fermion-arc-spectral}{{S22.6}{70}{The evolution along an arc and the quantum thimbles}{}{}}
\newlabel{sec:S-fermion-chain}{{S22.6}{71}{From the fermionic trace to one-dimensional quantum mechanics}{}{}}
\newlabel{sec:S-fermion}{{S23}{71}{The fermionic trace: the odd ensemble, the spectral equation and tests}{}{}}
\newlabel{eq:3d-half-turn}{{S23.1}{72}{The odd ensemble}{}{}}
\newlabel{eq:fermion-normal-currents}{{S23.2}{72}{The odd ensemble}{}{}}
\newlabel{sec:S-odd-cond}{{S23.2}{72}{The odd ensemble: the conditional correlation in the limit}{}{}}
\newlabel{eq:S-odd-orders}{{S23.3}{73}{The two orders}{}{}}
\newlabel{eq:S-odd-measure}{{S23.4}{74}{The half-turn measure}{}{}}
\newlabel{eq:S-odd-ZG}{{S23.5}{74}{The half-turn measure}{}{}}
\newlabel{eq:S-odd-small}{{S23.6}{75}{Small separation}{}{}}
\newlabel{eq:S-odd-small-h}{{S23.7}{75}{Small separation}{}{}}
\newlabel{eq:S-odd-gauss}{{S23.8}{76}{The spectrum at a fixed projected separation}{}{}}
\newlabel{eq:S-odd-plateau}{{S23.9}{76}{The spectrum at a fixed separation}{}{}}
\newlabel{eq:fermion-monodromy}{{S23.10}{77}{The spectrum of the transfer operator}{}{}}
\newlabel{eq:fermion-spectral}{{S23.11}{77}{The spectrum of the transfer operator}{}{}}
\newlabel{rem:fermion-bethe}{{S23.1}{78}{Is there a Bethe ansatz?}{}{}}
\newlabel{eq:3d-planar-identity}{{S23.12}{78}{The planar insertion}{}{}}
\newlabel{eq:fermion-planar-jump}{{S23.13}{78}{The planar insertion}{}{}}
\newlabel{eq:3d-one-label}{{S23.14}{78}{The planar insertion}{}{}}
\newlabel{eq:3d-parity-average}{{S23.15}{78}{The planar insertion}{}{}}
\newlabel{eq:3d-vertex-operators}{{S23.16}{78}{The planar insertion}{}{}}
\newlabel{sec:S-even-steps}{{S24}{79}{The source function of the even ensemble, step by step}{}{}}
\newlabel{eq:ev-pendulum}{{S24.1}{81}{Step 3: the hairpin factor becomes two pendulums}{}{}}
\newlabel{eq:S-ev-bands}{{S24.2}{83}{Step 9: the result}{}{}}
\newlabel{sec:S-even-arith-steps}{{S24.11}{84}{The labels near $\beta =\pi $}{}{}}
\newlabel{eq:ev-density}{{S24.3}{84}{The labels near $\beta =\pi $}{}{}}
\newlabel{sec:S-floquet-steps}{{S24.12}{84}{The Floquet form, step by step}{}{}}
\newlabel{eq:ev-split}{{S24.4}{84}{First: the square of a sum of two energies is an integral over an imaginary energy}{}{}}
\newlabel{eq:ev-floquet-kernel}{{S24.5}{85}{Second: the integral over the Bloch angle is a trace on the whole line}{}{}}
\newlabel{eq:S-Z-floquet}{{S24.6}{85}{The partition function}{}{}}
\newlabel{sec:S-asym-steps}{{S24.13}{86}{The asymptotes of the source}{}{}}
\newlabel{eq:S-end-a}{{S24.7}{86}{The end layers as quadratures}{}{}}
\newlabel{eq:S-end-p}{{S24.8}{86}{The end layers as quadratures}{}{}}
\newlabel{sec:pendulum}{{S25}{88}{The quantum pendulum: bands, Bloch states and the source}{}{}}
\newlabel{eq:pend-H}{{S25.1}{88}{Bands and Bloch states}{}{}}
\newlabel{eq:3d-fourier-matrix}{{S25.2}{88}{Bands and Bloch states}{}{}}
\newlabel{eq:pend-deep}{{S25.3}{88}{Bands and Bloch states}{}{}}
\newlabel{fig:pendulum}{{S1}{89}{The pendulum \eqref {eq:pend-H}. (a) The bands $\lambda _m(\alpha )$, $0\le \alpha \le 1$ (shaded, $m=0,\dots ,9$), against $\omega _L=h/4L$, with the barrier $\omega _L^2/2$ (dashed) and the deep-well levels \eqref {eq:pend-deep} (dotted). (b) The Bloch densities $|\psi _{m,\alpha }(\theta )|^2$ of the four lowest bands at $\omega _L=4$, at $\alpha =0$ (solid) and $\alpha =1$ (dashed), shifted vertically; the potential is shown below. The two lowest states lie below the barrier and are localized in the wells; the third is at the barrier, and the fourth is extended}{}{}}
\newlabel{eq:pend-bessel}{{S25.4}{89}{Matrix elements of the tip operators}{}{}}
\newlabel{eq:pend-duhamel}{{S25.5}{90}{The mean-field part}{}{}}
\newlabel{eq:pend-Sf}{{S25.6}{90}{The mean-field part}{}{}}
\newlabel{sec:pend-deep}{{S25.4}{90}{Deep wells}{}{}}
\newlabel{rem:3d-tba}{{S25.1}{91}{Exact WKB, the Mathieu TBA and Baxter's equation}{}{}}
\newlabel{sec:pend-floquet}{{S25.5}{91}{The Floquet form of the source}{}{}}
\newlabel{eq:pf-SB}{{S25.7}{91}{The Floquet form of the source}{}{}}
\newlabel{eq:pf-D}{{S25.8}{92}{The Floquet form of the source}{}{}}
\newlabel{eq:pf-T}{{S25.9}{92}{The Floquet form of the source}{}{}}
\newlabel{eq:pf-cell}{{S25.10}{92}{The Bloch angle}{}{}}
\newlabel{eq:pf-floquet}{{S25.11}{92}{The Bloch angle}{}{}}
\newlabel{eq:pf-Z-sum}{{S25.12}{93}{The cell trace of the partition function}{}{}}
\newlabel{eq:pf-riccati-kernel}{{S25.13}{93}{The cell trace of the partition function}{}{}}
\newlabel{eq:pf-Z-riccati}{{S25.14}{93}{The cell trace of the partition function}{}{}}
\newlabel{eq:pf-J-riccati}{{S25.15}{93}{The cell trace of the partition function}{}{}}
\newlabel{sec:S-cond}{{S26}{95}{The conditional state of the hairpin: formulas and checks}{}{}}
\newlabel{sec:S-cond-main}{{S26.1}{95}{The Gibbs state: the kind of theory, the gauge of the thermostat and the numerator}{}{}}
\newlabel{sec:S-cond-checks}{{S26.2}{96}{The partition function of the hairpin}{}{}}
\newlabel{eq:S-cond-path}{{S26.1}{97}{The path measure}{}{}}
\newlabel{eq:S-cond-free}{{S26.2}{98}{Small $h$}{}{}}
\newlabel{eq:cond-resolvent}{{S26.3}{98}{The endpoint operators}{}{}}
\newlabel{eq:cond-kernel}{{S26.4}{99}{The cell formula}{}{}}
\newlabel{eq:cond-cell}{{S26.5}{99}{The cell formula}{}{}}
\newlabel{eq:S-cond-large}{{S26.6}{99}{Values and asymptotes}{}{}}
\newlabel{sec:S-cond-literal}{{S26.3}{100}{The literal conditioning}{}{}}
\newlabel{eq:S-cond-bulk}{{S26.7}{101}{The bulk at finite $N$}{}{}}
\newlabel{sec:S-even-formulas}{{S27}{102}{The even ensemble at zero winding: explicit formulas}{}{}}
\newlabel{eq:ev-PQ}{{S27.1}{102}{The operators}{}{}}
\newlabel{eq:ev-spin-ops}{{S27.2}{102}{The operators}{}{}}
\newlabel{eq:ev-S2}{{S27.3}{103}{The operators}{}{}}
\newlabel{eq:ev-small-ratio}{{S27.4}{103}{Small $h$}{}{}}
\newlabel{sec:S-even}{{S28}{103}{The even ensemble at zero winding: exact sums and tests}{}{}}
\newlabel{sec:S-labels}{{S28.1}{103}{The sum over the rational angles}{}{}}
\newlabel{sec:S-valid}{{S28.2}{104}{Test of the continuum formula}{}{}}
\newlabel{sec:S-arith}{{S29}{104}{The arithmetic at zero winding}{}{}}
\newlabel{eq:ev-perron}{{S29.1}{105}{The arithmetic at zero winding}{}{}}
\newlabel{rem:ev-zeros}{{S29.1}{105}{Where the Riemann zeros go}{}{}}
\newlabel{eq:ev-theta}{{S29.2}{105}{Where the Riemann zeros go}{}{}}
\newlabel{fig:ev-arith}{{S2}{106}{The arithmetic of the zero-winding labels. (a) The density of labels near $\beta =\pi $, in units of its mean, against $X=N|\beta -\pi |/\pi $: the totient staircase \eqref {eq:ev-density} (line) and the exact labels at $N=20000$ in bins of width $0.1$ (circles); in the limit only the flat mean survives. (b) The finite-$N$ form factor of Remark~\ref {rem:ev-zeros} after subtraction of its real poles, $[R(t)-1-\pi ^2t/18-\dots ]/t^{3/4}$ (circles), and the contribution of the nontrivial zeros of $\zeta $ (line), dominated by the first zero}{}{}}
\newlabel{eq:ev-Rmellin}{{S29.3}{106}{Where the Riemann zeros go}{}{}}
\newlabel{sec:ev-eval}{{S30}{106}{Evaluation of the source function}{}{}}
\newlabel{sec:S-even-details}{{S31}{108}{The even ensemble at zero winding: details}{}{}}
\newlabel{fig:ev-G0}{{S3}{111}{The conditional source $C(h)=g/\Pi $ (solid), in units of $1/N$, with its numerator $g=h\widehat G$ (dashed) and the partition function $\Pi =h\widehat Z$ (dash-dotted), against $h$ on a logarithmic axis, $10^{-3}\le h\le 10^3$, with a linear vertical axis: lines through the Floquet quadratures \eqref {eq:ev-floquet} and \eqref {eq:cond-floquet}. Dotted: the limits $\frac 18$, $\sqrt \pi /32$ and $\sqrt \pi /4$ as $h\to 0$. Thin solid lines: the laws $C\simeq \frac 18-(4a_{1/2}/\sqrt \pi )h^{1/2}$ at small $h$, Eq.~\eqref {eq:ev-small}, and $\Pi \simeq (\log h+\bar \kappa )/(4\sqrt {2\pi })+c_0/h$ at large $h$, Eq.~\eqref {eq:ev-large}. Inset: $10^4\,C(h)$ on $1.2<h<2.5$, with linear axes and the line $C=0$; $C$ is negative on $\QCDIPLO <h<\QCDIPHI $, with the minimum $\QCMIN $ at $h\simeq \QCMINH $; the open circles mark the zeros and the dot the minimum}{}{}}
\newlabel{eq:ev-small-a}{{S31.1}{112}{Small $h$}{}{}}
\newlabel{sec:S-tail-closed}{{S31.4}{113}{Closed forms of the large-\texorpdfstring {$h$}{h} constants}{}{}}
\newlabel{eq:S-tail-closed}{{S31.2}{113}{Closed forms of the large-\texorpdfstring {$h$}{h} constants}{}{}}
\newlabel{eq:S-tail-closed-a2}{{S31.3}{113}{Closed forms of the large-\texorpdfstring {$h$}{h} constants}{}{}}
\newlabel{tab:S-tail-closed}{{S1}{114}{The closed forms \eqref {eq:S-tail-closed} and \eqref {eq:S-tail-closed-a2} of Ref.~\cite {JiangMigdalLean2026} against the values fitted to the Floquet values in this paper}{}{}}
\newlabel{sec:S-whole-evidence}{{S31.5}{114}{The evidence over the whole ensemble}{}{}}
\newlabel{sec:ev-whole}{{S32}{115}{The whole ensemble}{}{}}
\newlabel{sec:S-mc}{{S33}{116}{Direct simulation of the ensemble by a Markov chain}{}{}}
\newlabel{eq:mc-markov}{{S33.1}{117}{The algorithm}{}{}}
\newlabel{eq:mc-estimator}{{S33.2}{117}{The algorithm}{}{}}
\newlabel{sec:S-finiteN}{{S34}{119}{The finite-$N$ test of the conditional ratio}{}{}}
\newlabel{eq:S-finiteN-limits}{{S34.1}{119}{The finite-$N$ test of the conditional ratio}{}{}}
\newlabel{sec:S-finiteN-proof}{{S34.1}{123}{A proof of the limits}{}{}}
\newlabel{eq:S-fp-theorem}{{S34.2}{123}{A proof of the limits}{}{}}
\newlabel{eq:S-fp-pairs}{{S34.3}{123}{Pairs of spins}{}{}}
\newlabel{eq:S-fp-martingale}{{S34.4}{123}{Pairs of spins}{}{}}
\newlabel{eq:S-fp-trace}{{S34.5}{124}{From the walk to the pendulums}{}{}}
\newlabel{eq:S-fp-lower}{{S34.6}{124}{The pendulum integral}{}{}}
\newlabel{sec:S-spectrum-details}{{S35}{125}{The energy spectrum: details}{}{}}
\newlabel{sec:S-renorm}{{S35.1}{125}{Renormalization and the turbulent viscosity}{}{}}
\newlabel{eq:3d-renorm}{{S35.1}{126}{The renormalization}{}{}}
\newlabel{sec:S-weak-limit}{{S35.2}{129}{The weak limit and the chain of quadratures}{}{}}
\newlabel{eq:ev-weak-limit}{{S35.2}{129}{The weak limit and the chain of quadratures}{}{}}
\newlabel{eq:ev-chain}{{S35.3}{130}{The weak limit and the chain of quadratures}{}{}}
\newlabel{eq:ev-IR-next}{{S35.4}{131}{Infrared}{}{}}
\newlabel{sec:ev-mellin}{{S35.4}{133}{The Mellin amplitude}{}{}}
\newlabel{eq:ev-mellin}{{S35.5}{133}{The Mellin amplitude}{}{}}
\newlabel{eq:3d-energy-above-k0}{{S35.6}{134}{Time dependence: the energy above a fixed wave number}{}{}}
\newlabel{eq:3d-decay-index}{{S35.7}{135}{Time dependence: the energy above a fixed wave number}{}{}}
\newlabel{sec:S-energy-balance}{{S35.6}{135}{The energy balance}{}{}}
\newlabel{eq:S-balance}{{S35.8}{135}{The energy balance}{}{}}
\newlabel{eq:S-KH}{{S35.9}{136}{The Kolmogorov tensor}{}{}}
\newlabel{sec:S-open}{{S36}{137}{What remains to be settled}{}{}}
\newlabel{rem:3d-dissipation}{{S36.1}{137}{The dissipation lies outside the limit at fixed $K$}{}{}}
\newlabel{eq:3d-bulk-dissipation}{{S36.1}{137}{The dissipation lies outside the limit at fixed $K$}{}{}}
\newlabel{rem:3d-energy-normalization}{{S36.2}{138}{Energy normalization is postponed}{}{}}
\newlabel{rem:3d-matching}{{S36.3}{138}{Convergence and matching}{}{}}
\newlabel{rem:ev-open}{{S36.4}{138}{What the conditional spectrum rests on}{}{}}
\newlabel{sec:S-spectrum}{{S37}{139}{The spectrum: selected values and accuracy}{}{}}
\newlabel{sec:S-annealed}{{S37.1}{140}{The annealed order: the spectrum, the correlation and the finite-size effects}{}{}}
\newlabel{eq:S-ann-c}{{S37.1}{140}{The correlation}{}{}}
\newlabel{eq:S-ann-small}{{S37.2}{140}{The correlation}{}{}}
\newlabel{eq:S-ann-large}{{S37.3}{141}{The correlation}{}{}}
\newlabel{eq:S-ann-P}{{S37.4}{141}{The transform}{}{}}
\newlabel{eq:S-ann-IR}{{S37.5}{142}{The laws}{}{}}
\newlabel{eq:S-ann-I}{{S37.6}{143}{Finite size}{}{}}
\newlabel{sec:S-osc-derivation}{{S38}{144}{Oscillations in coordinate space: derivations}{}{}}
\newlabel{eq:osc-source-cond}{{S38.1}{145}{The amplitude}{}{}}
\newlabel{eq:osc-a2}{{S38.2}{145}{The amplitude}{}{}}
\newlabel{eq:osc-lighthill}{{S38.3}{145}{The amplitude}{}{}}
\newlabel{eq:osc-mellin}{{S38.4}{146}{Small separation}{}{}}
\newlabel{fig:osc-index}{{S4}{148}{Effective indices of the correlation functions of the conditional state, against $\log (r/L)$. (a) The index $n_\omega =-\partial \log C_\omega /\partial \log r$ of the vorticity correlation (line); the same with the oscillating term of the source removed (dashed), and the envelope $n_\omega ^{\rm reg}\pm 2\sqrt \pi \,|D|/[\Pi (R/\sqrt 2)\,R^2c_{\rm reg}(R)]$ of the oscillation, Eq.~\eqref {eq:osc-n} (dotted), both for $r\ge 4\sqrt 2\,L$: the oscillating term is removed for $h>2$, fully from $h=4$, and the Abel average reaches $h=R/\sqrt 2$. The horizontal line marks $2$. The oscillation decays asymptotically as $1/\log ^2(r/L)$. (b) The index $\zeta _2$ of the velocity structure function \eqref {eq:osc-zeta} (line); its small-$R$ law $2-\QCOZSMALL \,R^{1/2}$ (dashed); its large-$R$ law, the first relation of \eqref {eq:osc-S-large} divided by its integral, with the constant of integration taken from the computed $\mathcal S$ at $R=10^4$ (dotted); the asymptote $2/\log R$, which is reached only logarithmically (thin dotted); and the index $\zeta _{LL}$ of the longitudinal function (dash-dotted). The horizontal line marks $2/3$}{}{}}
\newlabel{eq:osc-DC}{{S38.5}{149}{The velocity structure function}{}{}}
\newlabel{eq:osc-zeta-osc}{{S38.6}{149}{The velocity structure function}{}{}}
\newlabel{sec:S-osc}{{S39}{150}{Oscillations in coordinate space: computations}{}{}}
\newlabel{fig:osc-origin}{{S5}{151}{The origin of the wave. (a) The oscillating part of the source, $h^{5/2}[h\widehat G-s(h)]$ with $s$ the fitted non-oscillating part of \eqref {eq:ev-large}, with its next orders in $1/h$, for the computed values $6\le h\le 80$, divided by its amplitude $|D_{\rm eff}|$ and plotted against its phase $\phi $ modulo $2\pi $: open circles with the stationary-phase amplitude of \eqref {eq:osc-source}, $D_{\rm eff}=D$ and $\phi =2h+\arg D$; filled circles, coloured by $\log h$, with the next order, $D_{\rm eff}=D+D_1/h$; the line is $\cos \phi $. (b) The oscillating part of the conditional vorticity correlation \eqref {eq:ev-corr}, in units of $10^{-3}$: the difference between the correlations computed with the full source and with its oscillating part removed, multiplied by $R^3\,h\widehat Z(h)$ at $h=R/\sqrt 2$, minus its average over one period (line), the asymptotic form \eqref {eq:osc-c} (dashed), and the same with $D+\sqrt 2D_1/R$ in place of $D$ (dotted); the removal is complete for $r>4\sqrt 2\,L$, and for $R\ge 6$ the subtraction of the non-oscillating part computed from the moments of the removed term, as in the table of this section, gives the same curve to about $2\%$ of $|D|$. The period is $\pi $ in $h$ and $2\pi /\sqrt 2$ in $R=r/L$: the Abel integral reads the source, and the partition function, at $h=R/\sqrt 2$}{}{}}
\newlabel{sec:S-limits-full}{{S40}{152}{The scaling limits: layers, exponents and the choice}{}{}}
\newlabel{sec:S-limits}{{S41}{154}{The scaling limits of the even ensemble}{}{}}
\newlabel{eq:S-lim-s2}{{S41.1}{155}{The Gaussian layer}{}{}}
\newlabel{eq:S-lim-clt}{{S41.2}{155}{The Gaussian layer}{}{}}
\newlabel{eq:lim-P1}{{S41.3}{155}{The function $P_1$}{}{}}
\newlabel{eq:lim-F}{{S41.4}{155}{The function $P_1$}{}{}}
\newlabel{eq:lim-P1-asym}{{S41.5}{155}{The function $P_1$}{}{}}
\newlabel{eq:S-lim-VN}{{S41.6}{156}{The function $P_1$}{}{}}
\newlabel{eq:S-lim-Fuv}{{S41.7}{156}{The function $P_1$}{}{}}
\newlabel{sec:S-small-angles}{{S42}{158}{The small-angle layer is exponentially small}{}{}}
\newlabel{eq:S-sa-E}{{S42.1}{158}{The result}{}{}}
\newlabel{sec:S-sa-mirror}{{S42.1}{158}{The mirror symmetry \texorpdfstring {$\beta \to 2\pi -\beta $}{beta -> 2 pi - beta}}{}{}}
\newlabel{eq:S-sa-mirror}{{S42.2}{158}{The mirror symmetry \texorpdfstring {$\beta \to 2\pi -\beta $}{beta -> 2 pi - beta}}{}{}}
\newlabel{eq:S-sa-label}{{S42.3}{159}{One label}{}{}}
\newlabel{eq:S-sa-arc}{{S42.4}{159}{The arc operators}{}{}}
\newlabel{eq:S-sa-decay}{{S42.5}{159}{The arc operators}{}{}}
\newlabel{prop:S-sa-reduction}{{S42.1}{159}{Reduction to single arcs}{}{}}
\newlabel{eq:S-sa-bound}{{S42.6}{159}{Reduction to single arcs}{}{}}
\newlabel{eq:S-sa-layer}{{S42.7}{160}{Consequences}{}{}}
\newlabel{sec:S-sa-arcs}{{S42.3}{161}{The decay along one arc}{}{}}
\newlabel{prop:S-sa-arcs}{{S42.2}{161}{One arc}{}{}}
\newlabel{sec:S-sa-numerics}{{S42.5}{163}{Numerical checks}{}{}}
\newlabel{fig:S-small-angles}{{S6}{165}{The small-angle layer. (a) The arc operator on the lattice: $-\log \rho (T_\lambda )/\gamma _0$ against $\beta \sqrt \lambda $ at fixed $\lambda \beta $. (b) $\sum |W_{N,p/q}|$ over the layer $\beta \le 3/\sqrt N$ (points) and the whole source $W_N(h)$ (lines). (c) Every small-angle label computed: $\log _{10}|W_{N,p/q}|$ against $E_{p/q}/2$, Eq.~\eqref {eq:S-sa-E}; dashed: $e^{-3.7-E_{p/q}/2}$}{}{}}
\newlabel{sec:S-discussion}{{S43}{165}{The Conclusion in full}{}{}}
\newlabel{sec:S-code}{{S44}{172}{Computational material}{}{}}
\makeatother

